Beyond Traditional Neural Networks: Toward adding Reasoning and Learning Capabilities through Computational Logic Techniques

Deep Learning (DL) models have become popular for solving complex problems, but they have limitations such as the need for high-quality training data, lack of transparency, and robustness issues. Neuro-Symbolic AI has emerged as a promising approach combining the strengths of neural networks and symbolic reasoning. Symbolic knowledge injection (SKI) techniques are a popular method to incorporate symbolic knowledge into sub-symbolic systems. This work proposes solutions to improve the knowledge injection process and integrate elements of ML and logic into multi-agent systems (MAS).

==> eptcsdata.tex <==
\providecommand{\firstpage}{416}
\providecommand{\publicationstatus}{S. Costantini, E. Pontelli, A. Russo, F. Toni,\\R. Calegari, A. D'Avila Garcez, C. Dodaro, F. Fabiano,\\ S. Gaggl, A. Mileo, (Eds.): ICLP 2023\\
EPTCS 385, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.385.51}{10.4204/EPTCS.385.51}}

